Leveraging Structured Biological Knowledge for Counterfactual Inference: a Case Study of Viral Pathogenesis

Counterfactual inference is a useful tool for comparing outcomes of interventions on complex systems. It requires us to represent the system in form of a structural causal model, complete with a causal diagram, probabilistic assumptions on exogenous variables, and functional assignments. Specifying such models can be extremely difficult in practice. The process requires substantial domain expertise, and does not scale easily to large systems, multiple systems, or novel system modifications. At the same time, many application domains, such as molecular biology, are rich in structured causal knowledge that is qualitative in nature. This manuscript proposes a general approach for querying a causal biological knowledge graph, and converting the qualitative result into a quantitative structural causal model that can learn from data to answer the question. We demonstrate the feasibility, accuracy and versatility of this approach using two case studies in systems biology. The first demonstrates the appropriateness of the underlying assumptions and the accuracy of the results. The second demonstrates the versatility of the approach by querying a knowledge base for the molecular determinants of a severe acute respiratory syndrome coronavirus 2 (SARS-CoV-2)-induced cytokine storm, and performing counterfactual inference to estimate the causal effect of medical countermeasures for severely ill patients.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> arxiv submission/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> arxiv submission/acronyms.tex <==

\DeclareAcronym{ett}{
    short = ETT,
    alt   = \text{ETT},
    long  = effect of the treatment on the treated.
}

\DeclareAcronym{ite}{
    short = ITE,
    alt   = \text{ITE},
    long  = individual treatment effect
}

\DeclareAcronym{ate}{
    short = ATE,
    alt   = \text{ATE},
    long  = average treatment effect
}

\DeclareAcronym{raf}{
    short = RAF,
    alt   = \text{RAF},
    long  = Rapidly Accelerated Fibrosarcoma
}
\DeclareAcronym{mek}{
    short = MEK,
    alt   = \text{MEK},
    long  = MAPK ERK kinase,
}
\DeclareAcronym{erk}{
    short = ERK,
    alt   = \text{ERK},
    long  = Extracellular signal-regulated kinases,
}
\DeclareAcronym{toci}{
    short = Toci,
    alt   = \text{Toci},
    long  = Tocilizumab,
}

\DeclareAcronym{prr}{
    short = PRR,
    alt   = \text{PRR},
    long  = Pathogen Recognition Receptors,
}

\DeclareAcronym{ace2}{
    short = ACE2,
    alt   = \text{ACE2},
    long  = Angiotensin Converting Enzyme 2,
}

\DeclareAcronym{agtr1}{
    short = AGTR1,
    alt   = \text{AGTR1},
    long  = Angiotensin II Receptor 1,
}


\DeclareAcronym{adam17}{
    short = ADAM17,
    alt   = \text{ADAM17},
    long  = A Disintegrin And Metalloproteinase 17,
}
\DeclareAcronym{tnf}{
    short = TNF$\alpha$,
    alt   = \text{TNF$\alpha$},
    long  = Tumor Necrosis Factor $\alpha$,
}
\DeclareAcronym{il6stat3}{
    short = IL6-STAT3,
    alt   = \text{IL6-STAT3},
    long  = Interleukin 6 STAT3 Complex,
}

\DeclareAcronym{egf}{
    short = EGF,
    alt   = \text{EGF},
    long  = Epidermal Growth Factor,
}
\DeclareAcronym{ards}{
    short = cytokine storm,
    alt   = \text{CytokineStorm},
    long  = Cytokine Release Syndrome
}
\DeclareAcronym{nfkb}{
    short = NF-$\kappa$B,
    alt   = \text{NF-$\kappa$B},
    long  = nuclear factor kappa-light-chain-enhancer of activated B cell,
}
\DeclareAcronym{il6r}{
    short = mIL6R,
    long  = membrane-bound Interleukin 6 receptor,
}
\DeclareAcronym{sil6r}{
    short = sIL6R$\alpha$,
    alt   = \text{sIL6R$\alpha$},
    long  = soluble Interleukin 6 receptor,
}
\DeclareAcronym{il6amp}{
    short = IL6-AMP,
    alt   = \text{IL6-AMP},
    long  = Interleukin 6 Amplifier,
}
\DeclareAcronym{il6}{
    short = IL6,
    alt   = \text{IL6},
    long  = Interleukin 6,
}
\DeclareAcronym{il6st}{
    short = IL6ST,
    alt   = \text{IL6ST},
    long  = Interleukin 6 Signal Transducer
}

\DeclareAcronym{stat3}{
    short = STAT3,
    alt   = \text{STAT3},
    long  = Signal Transducer and Activator of Transcription 3,
}



\DeclareAcronym{egfr}{
    short = EGFR,
    alt   = \text{EGFR},
    long  = Epidermal Growth Factor Receptor,
}

\DeclareAcronym{sars2}{
    short = SARS-CoV-2,
    alt   = \text{SARS-CoV-2},
    long  = severe acute respiratory syndrome coronavirus 2,
}

\DeclareAcronym{bionlp}{
    short = BioNLP,
    long  = natural language processing of biomedical literature
}

\DeclareAcronym{ang}{
    short = Angiotensin II,
    alt   = \text{Angiotensin II},
    long  = Angiotensin II,
}

\DeclareAcronym{AF}{
    short = AF,
    long  = Activity Flow,
    long-plural-form = Activity Flows,
    cite  = le2009systems,
}
\DeclareAcronym{sbml}{
    short = SBML,
    long  = Systems Biology Markup Language,
    cite  = hucka2018systems,
}

\DeclareAcronym{qual}{
    short = SBML-qual,
    long  = \ac{sbml} Qualitative Models Package,
    cite  = chaouiya_2013,
}

\DeclareAcronym{biopax}{
    short = BioPAX,
    long  = Biological Pathway Exchange Language,
    cite  = demir_2010,
}
\DeclareAcronym{BEL}{
    short = BEL,
    long  = Biological Expression Language,
    cite  = Slater2014,
}
\DeclareAcronym{covid19}{
    short = COVID-19,
    long  = coronavirus disease 2019
}
\DeclareAcronym{igf}{
    short = IGF,
    long  = insulin-like growth factor
}
\DeclareAcronym{INDRA}{
    short = INDRA,
    long  = Integrated Dynamical Reasoner and Assembler,
    cite  = gyori2017word,
}
\DeclareAcronym{ODE}{
    short = ODE,
    short-plural-form = ODEs,
    long  = ordinary differential equation,
    long-plural-form = ordinary differential equations,
}
\DeclareAcronym{PDE}{
    short = PDE,
    long  = partial differential equation,
    long-plural-form = partial differential equations,
}
\DeclareAcronym{NFKB}{
    short = NF-$\kappa$B,
    long  = nuclear factor kappa-light-chain-enhancer of activated B cells,
}
\DeclareAcronym{NPA}{
    short = NPA,
    long  = Network Perturbation Amplitude,
    cite  = Martin2014
}
\DeclareAcronym{MAPK}{
    short = MAPK,
    long  = mitogen-activated protein kinase,
}
\DeclareAcronym{mRNA}{
    short = mRNA,
    long  = messenger ribonucleic acid,
    long-plural-form = messenger ribonucleic acids,
}
\DeclareAcronym{PD}{
    short = PD,
    long  = Process Description,
    long-plural-form = Process Descriptions,
    cite  = le2009systems,
}
\DeclareAcronym{RCR}{
    short = RCR,
    long  = Reverse Causal Reasoning,
    cite  = Catlett2013
}
\DeclareAcronym{sarscov2}{
    short = SARS-CoV-2,
    long  = severe acute respiratory syndrome coronavirus 2
}
\DeclareAcronym{SBGN}{
    short = SBGN,
    long  = Systems Biology Graphical Notation,
    cite  = le2009systems,
}

\DeclareAcronym{SCM}{
    short            = SCM,
    long             = structural causal model,
    long-plural-form = structural causal models,
}
\DeclareAcronym{SDE}{
    short = SDE,
    long  = stochastic differential equation,
    long-plural-form = stochastic differential equations,
}
\DeclareAcronym{bel2scm}{
    short = \textsc{bel2scm},
    long  = Biological Expression Language to Structural Causal Models,
    alt   = https://github.com/bel2scm
}     
\DeclareAcronym{query2bel}{
    short = \textsc{query2bel},
    long  = Causal query to Biological Expression Language,
    alt   = https://github.com/bel2scm
}     

\DeclareAcronym{cord19}{
    short = CORD-19,
    long  = COVID-19 Open Research Dataset,
    cite  = luwang_2020,
}     

\DeclareAcronym{biodati}{
    short = BioDati,
    long  = BioDati Inc.,
}
\DeclareAcronym{covid19kg}{
    short = Covid19kg,
    long  = Fraunhofer Covid-19 Knowledge Graph,
}
\DeclareAcronym{sigscm}{
    short = $\aca{SCM}^\sigma$,
    long  = sigmoidal \acl{SCM}
}
\DeclareAcronym{mmscm}{
    short = $\aca{SCM}^{MM}$,
    long  = \acl{SCM} with a Michaelis-Menten functional form
}



==> arxiv submission/background.tex <==
\noindent {\textbf{Biological signaling pathways}}
Signaling pathways are composed of entities that engage in activities~\cite{machamer_2000}.
Examples of entities are proteins and metabolites, but also higher level biological processes such as an immune response.
Activities are the producers of change.
Examples include catalytic activity, kinase activity, or transcriptional activity.

The basic unit of causality in signaling pathways is a directed molecular interaction, where the activity of an upstream molecule increases or decreases the activity of a downstream molecule. 
For example, the \acf{MAPK} intracellular signaling pathway is a causal chain of directed molecular interactions shown  in~\eqref{mapkNet} 
\begin{eqnarray}
    \label{mapkNet}
    a(S_1) \rightarrow kin(p(Raf)) \rightarrow kin(p(Mek)) \rightarrow kin(p(Erk))
\end{eqnarray}
The interactions transmit information about a stimulus at the cell surface to the nucleus, where proteins called transcription factors activate an appropriate biological process~\cite{Li2017}.  
A causal diagram of \ac{MAPK} consists of a signaling molecule $S_1$ and three proteins $Raf$, $Mek$, and $Erk$, each of which engage in kinase activity.
We represent signaling molecule abundance with $a()$, protein abundance with $p()$ and the kinase activity of a protein with $kin()$.
In the case of MAPK, the abundance or activity of an upstream entity causes the abundance or activity of a downstream entity to increase, and is represented with a sharp edge $\rightarrow$.
The diagram is a abstraction showing that the abundance of the signaling molecule  $S_1$ increases the kinase activity of $Raf$, which increases the kinase activity of $Mek$, which increases the kinase activity of $Erk$. 
In other cases, if the abundance or activity of an upstream entity causes the abundance or activity of a downstream entity to decrease, we represent this with a blunt edge $\rightinhibits$.


\medskip \noindent {\textbf{Viral dysregulation}}
Viral disruptions of a signaling pathway take form of overactivation or repression of its activities.
%This can be a side effect of exploiting cellular machinery that\textemdash while detrimental to the infected host\textemdash has minimal benefit or cost to the virus, or it can be an evolved function of the virus that in some way enhances the viral lifecycle.
%Infection and viral reproduction are cellular level phenomenon, but disease is a system-level phenomenon, which includes both the direct damage the virus does to individual cells as well as the totality of the cellular damage incurred by the immune response to the virus.
%Just like a cellular-level response is regulated by intracellular signaling pathways, the system-level immune response is regulated by intercellular signaling pathways.
%Viruses can also dysregulate these intercellular signaling pathways. 
For example, by amplifying the release of intercellular signaling molecules that overstimulate the immune response, known as \acf{ards}, a virus can cause severe system-level cellular damage.

\medskip \noindent {\textbf{Quantitative modeling of biological processes with ODE/SDE}}
Temporal dynamics of biological processes can be expressed quantitatively using ordinary (or stochastic) differential equations.
A small number of high quality, validated models have been published in the literature and stored in a computable form in repositories such as Biomodels~\cite{chen2010modeling,gratie2013ode}.
For example, the \ac{MAPK} signaling pathway in~\eqref{mapkNet} is well characterized. We denote $R(t)$, $M(t)$, and $E(t)$ as the respective amounts of active $Raf$, $Mek$, and $Erk$ at time $t$;
We denote $T_{R}$, $T_{M}$, and $T_{E}$ as their total amounts, which we assume do not change during the considered timeframe;
$v^\text{act}_R$, $v^\text{inh}_R$, $v^\text{act}_M$, $v^\text{inh}_M$, $v^\text{act}_E$, and $v^\text{inh}_E$ are experimentally derived activation or inhibition kinetic rate constants; and $S_1$ is the amount of the input signal.
The system of \acp{ODE} is specified as follows \cite{bianconi2012computational, kim2010pathological}:

\begin{small}
\label{mapkODE}
\begin{align}
        \label{mapkODE}
        \frac{\mathrm{d}R}{\mathrm{d}t} &= v^{\text{act}}_{R} S_1 (T_{R}-R(t)) - v^{\text{inh}}_{R}R(t)  \\
        \frac{\mathrm{d}M}{\mathrm{d}t} &=  \frac{(v^{\text{act}}_{M})^2}{v^{\text{inh}}_{M}}R(t)^2(T_{M} - M(t)) - v^{\text{act}}_{M}R(t)M(t) - v^{\text{inh}}_{M}M(t) \nonumber \\
        \frac{\mathrm{d}E}{\mathrm{d}t} &=  \frac{(v^{\text{act}}_{E})^2}{v^{\text{inh}}_{E}}M(t)^2(T_{E} - E(t)) - v^{\text{act}}_{E}M(t)E(t) - v^{\text{inh}}_{E}E(t) \nonumber
\end{align}
\end{small}

Given initial conditions, forward simulations from the \acp{ODE} can be used to generate the temporal trajectories of the amounts of activated proteins , such as $R(t)$, $M(t)$, and $E(t)$ in the \ac{MAPK} example.
In this manuscript we refer to such simulated data as \textit{observational data}.
We define an \textit{ideal intervention} as an event that fixes the amount of an activated protein.
For example, if we fix the kinase acivity of $Mek$ at $M(t) = m$, the second equality $\frac{\mathrm{d} M}{\mathrm{d} t}$ in~\eqref{mapkODE} becomes zero.
We can simulate data from \eqref{mapkODE} with $\frac{\mathrm{d} M}{\mathrm{d} t}=0$, and refer to these as \textit{interventional data}.
Contrasting observational and interventional data helps evaluate the outcome of the intervention~\cite{ness2019integrating}.

The deterministic \ac{ODE} ignore the fact that at low concentration, stochasticity becomes a significant factor in determining the reaction \cite{paneri2019integrating}.
As the collisions between molecules participating in biochemical process become stochastic, a stochastic model is required.
In contrast to \ac{ODE}, a stochastic differential equation model or \ac{SDE} specifies biological process as a random process.
For example, in the case of \ac{MAPK}, the random process of the reaction $Mek \rightarrow Erk$ is specified with
\begin{eqnarray}
\frac{dP_{E} (t)}{dt} = g_{E}(t, v^{act}_E, v^{inh}_E, M(t)),\  E(0) = e_0
\end{eqnarray}
where $P_E(t)$ is marginal probability density of $E(t)$, function $g_{E}$ determines the probability of a state change between $E(t)$ and $E(s), s > t$, $e_0$ is initial condition, and $M(t)$ is the value of its parent Mek at $t$.
Once \acl{SDE} are fully specified, one can use, e.g. Gillespie's stochastic simulation algorithm ~\cite{gillespie1977exact} to simulate observational and interventional data, and evaluate the outcomes of interventions.

Unfortunately, even simple \acp{ODE} such as the one in the \ac{MAPK} example are difficult to build \textit{de novo}. This is nearly impossible for novel and poorly studied systems that lack the existence or findability of experimental information describing the structure or boundaries of the process, kinetic equations governing their dynamics~\cite{jha2012exploring}, rate constants for these equations, or rules governing each agents' states and functions.

\medskip \noindent {\textbf{Equilibrium enzyme kinetics}} Simpler and more general quantitative models can be specified when a reaction reaches the state of chemical equilibrium~\cite{alon2019introduction}. One commonly used such model is \textit{Hill function} in the form of 
\begin{eqnarray}
X = \beta \frac{\mathbf{PA}_X^n}{K^n + \mathbf{PA}_X^n}
\end{eqnarray}
where $X$ is the abundance of a protein in a causal diagram (such as $Erk$ in~\eqref{mapkNet}), $\mathbf{PA}_X$ is the set of its parents, $n$ is a parameter interpreted as the number of ligand binding sites of the protein, and $\beta$ is the total number of molecules of the protein. A special and frequently used case of the Hill function, called \textit{Michaelis-Menten} function, occurs when $n=1$. Although simple to use, these models are deterministic, and do not describe the stochasticity that is a distinctive property of biological systems at low concentrations. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t!]
\centering
\begin{tabular}{ccc}
\scalebox{.7}{\tikz{
    % nodes
     \node[obs] (Raf) {$Raf$};%
     \node[obs,right=of Raf] (Mek) {$Mek$}; %
     \node[obs,right=of Mek] (Erk) {$Erk$}; %
     \node[latent,,rectangle,below=of Erk] (fErk) {$f_{Erk}$}; %
    \node[latent,,rectangle,below=of Mek] (fMek) {$f_{Mek}$}; %
    % hyperparameters
    \node[latent, below =of Raf] (NRaf) {$N_{Raf}$} ; %
    \node[latent, below =of fErk] (NErk) {$N_{Erk}$} ; %
    \node[latent, below =of fMek] (NMek) {$N_{Mek}$} ; %
    % edges
    \edge{Raf}{fMek};
     \edge {fMek}{Mek};
     \edge {Mek} {fErk};
     \edge{fErk} {Erk};
     \edge {NRaf}{Raf};
     \edge {NErk} {fErk};
     \edge {NMek} {fMek}
     }}& $~~~$ &
     \scalebox{.7}{\tikz{
    % nodes
     \node[latent] (Raf) {$Raf$};%
     \node[obs,accepting,right=of Raf] (Mek) {$m'$}; %
     \node[latent,right=of Mek] (Erk) {$Erk$}; %
     \node[latent,,rectangle,below=of Erk] (fErk) {$f_{Erk}$}; %
    % hyperparameters
    \node[latent, below =of Raf] (NRaf) {$\hat{N}_{Raf}$} ; %
   % \node[latent, below =of Mek] (NMek) {$N_{Mek}$} ; %
    \node[latent, below =of fErk] (NErk) {$\hat{N}_{Erk}$} ; %
   
    % edges
     \edge {Mek} {fErk};
     \edge{fErk} {Erk};
     \edge {NRaf}{Raf};
     \edge {NErk} {fErk};
      % \edge {NMek} {Mek};
     }}\\
     (a) & & (b)
\end{tabular}

\caption{\small \textbf{Causal modeling of MAPK signaling pathway} Circles are variables, double circles are variables intervened upon, squares are deterministic functional assignments, gray nodes are observed variables, and white nodes are hidden variables. (a) Structural causal model. $N_{Raf}$, $N_{Mek}$ and $N_{Erk}$ are statistically independent noise variables. Root node $Raf$ is only dependent on noise variable $N_{Raf}$. Non-root nodes $Mek$ and $Erk$ are dependent on their parent and on the associated noise variable. (b) Counterfactual model. The intervention fixes the count of phosphorylated $Mek$ to $m'$, such that $Mek$ is no longer dependent on $Raf$ and $N_{Mek}$. Given an observed data point, counterfactual inference infers the noise variables $\hat{N}_{Raf}$, and $\hat{N}_{Erk}$. \label{fig:mapkNet}}

\end{figure}



\medskip \noindent {\textbf{Modeling biological processes with structural causal models}}
The stochastic nature of biological processes at steady-state can be represented by an \ac{SCM} such as in ~\figref{fig:mapkNet} (a)~\cite{BongersMooij_1803.08784,ness2019integrating}.
\acp{SCM} represent the dependencies between a child node $X$ and its parents $\mathbf{PA}_X$ in terms of a deterministic function $X = f_X(\mathbf{PA}_X, N_X)$ called \textit{structural assignment}, and a noise variable $N_X$.
In~\figref{fig:mapkNet} (a), $f_{Mek}$ and $f_{Erk}$ are linear or non-linear structural assignments, and $N_{Raf}$, $N_{Mek}$, and $N_{Erk}$ are statistically independent noise variables with defined probability distributions
\begin{eqnarray}
Raf = N_{Raf};\ Mek = f_{Mek}(Raf ; N_{Mek})\\
Erk = f_{Erk}(Mek,N_{Erk}) \nonumber
\label{SCMBackground}
\end{eqnarray}
An ideal intervention in an \ac{SCM} is performed on a functional assignment. For example, an ideal intervention on $Mek$ sets $Mek = m^{\prime}$, defining a new \ac{SCM}
\begin{eqnarray}
    \label{IntervenedSCMBackground}
    & Raf = N_{Raf};  Mek = m^{\prime};  Erk = f_{Erk}(Mek,N_{Erk}) &
\end{eqnarray}
An ideal intervention can also be thought of as a process of mutilating the causal graph.
For example, intervening on $Mek$ eliminates its dependence upon $Raf$, and therefore the edge from $Raf$ to $Mek$ is removed as shown in \figref{fig:mapkNet}(b). 

\medskip \noindent {\textbf{Counterfactual inference with \ac{SCM}}
Beyond direct model-based predictions, \Acp{SCM} enable {\it counterfactual inference}, i.e., the process of inferring the unseen outcomes of a hypothetical intervention given data observed in absence of the intervention~\cite{pearl2009causal}.
In the context of \ac{SCM}, counterfactuals are defined as operations
\begin{eqnarray}
& Y_{do(T=t^{\prime})}(u) \triangleq Y_{M_{do(T=t^{\prime})}}(u) &
\end{eqnarray}
In other words, the outcome $Y$ that individual $u$ would have had she received treatment $t^{\prime}$ is defined as the value that $Y$ would have in a structural causal model $M$ mutilated to replace $T=f_T(\cdot)$ with $T=t^{\prime}$.

For example, in the MAPK signaling pathway, we may be interested in the counterfactual question: \textit{Having observed the kinase activities of  $Raf = r$, $Mek = m$, $Erk = e$, what would be the kinase activity of $Erk$ in a hypothetical experiment where the kinase activity of $Mek$ was fixed to $m^{\prime}$?}
This counterfactual query is more formally translated into
\begin{eqnarray}
    P (Erk_{do( Mek= m^{\prime})} | Raf = r, Mek = m, Erk = e) \label{eq:exampleCounterfactual}
\end{eqnarray}
The probability distribution in~\eqref{eq:exampleCounterfactual} is estimated with the following steps:
\begin{enumerate}
\item \textbf{Abduction:} Given observational data, estimate the posterior distribution of the noise variables.
In the MAPK example, we estimate the posterior distribution of the noise variables:
\begin{align*}\hat{N}_{Raf} = & \{N_{Raf} | Raf = r, Mek = m, Erk = r\} \\
\hat{N}_{Erk} = & \{N_{Erk} | Raf = r, Mek = m, Erk = r\}
\end{align*}
Several  inference algorithms are available for this task, e.g. Markov Chain Monte Carlo \cite{jerrum1997markov}, Gibbs sampling  \cite{gelfand2000gibbs}, or no-u-turn Hamiltoninan Monte Carlo (HMC)~\cite{hoffman2014no}.
In recent years, gradient-based inference algorithms such as stochastic variational inference \cite{hoffman2013stochastic} have become popular, because they can scale to larger models by converting an inference problem into an optimization problem.
\item \textbf{Intervention:} Apply the intervention to the SCM to generate a mutilated SCM as in~\figref{fig:mapkNet}(b). 
%%In the \ac{MAPK} \ac{SCM}, $\hat{N}_{Raf}$ and $\hat{N}_{Erk}$ are replaced with $N_{Raf}$ and $N_{Erk}$ as shown in \figref{fig:mapkNet}(a).
In the \ac{MAPK} \ac{SCM}, $Mek = f_{Mek}(Raf,N_{Mek})$ is replaced with $Mek=m'$ as shown in~\figref{fig:mapkNet}(b).
\item \textbf{Prediction:}  Generate samples from the mutilated SCM using the estimated posterior distribution over the exogenous variables $\hat{N}_{Raf}$ and $\hat{N}_{Erk}$  to obtain the counterfactual distribution, as shown in~\figref{fig:mapkNet}(b).
\end{enumerate}
\medskip \noindent {\textbf{Causal effects}}
We distinguish between two causal effects. The first is the \acf{ate}, defined as the difference between the outcome of a hypothetical intervention and the observed outcome in the entire population.
In the MAPK example, the ATE of $Erk$ upon an intervention fixing $Raf=r^{\prime}$ is:
\begin{eqnarray}
& \left\{Erk_{do(Raf= r^{\prime})}  - Erk  \right\} &
\end{eqnarray}
This requires no observational data, and therefore the \acf{ate} can be inferred with forward simulation.

On the other hand, the \acf{ite} is defined as the difference between the outcome of a hypothetical intervention and the observed outcome for a specific individual or context.
In the MAPK example, the \acl{ite} of $Erk$ upon an intervention fixing $Raf=r^{\prime}$ in a context where  $Raf = r$, $Mek = m$, $Erk = e$ is:
\begin{eqnarray}
\left\{Erk_{do(Raf= r^{\prime})}  - Erk  \right\} | Raf = r, Mek = m, Erk = e
\end{eqnarray}
The \ac{ite} shares stochastic components of the noise variables between observational and interventional data, and is therefore often more precise than a comparison based on a direct simulation~\cite{ness2019integrating}. 

In cases where domain knowledge is available to describe the systems dynamics in the form of an SDE, the system at equilibrium can be translated into an \ac{SCM} to enable counterfactual reasoning and estimation of the \acl{ite}~\cite{blom2018beyond,ness2019integrating}.
Unfortunately, this process is challenging in novel and poorly studied systems, due to our limited ability to establish the structure of the causal graph.

\medskip \noindent {\textbf{Structured knowledge graphs}}
Although there exist a multitude of biological knowledge bases that are manually curated from the literature~\cite{Cerami2011,Fabregat2018,Kanehisa2017,Perfetto2016,Slenter2018}, the systems biology community has coalesced around a small number of structured knowledge representations that differ mainly in their intended purpose.
For example, the \acf{biopax} was designed for pathway database integration~\cite{demir_2010}, and the \acf{SBGN} was designed for graphical layout~\cite{le2009systems}.

In contrast, the \acf{BEL} was specifically designed for manual extraction and automated integration of author statements about causal relationships  among biological entities, biological processes, and cellular-level observable phenomena~\cite{hoyt2019}.
The syntax of a BEL statement is comprised of a  triple in the form of \{\textit{subject}, \textit{predicate}, \textit{object}\}.
Each subject and object represents an activity or abundance whose entities are grounded using terms from  standard namespaces.
If the subject directly increases the abundance or the activity of the object, we represent this with \verb+=>+, and for directly decreasing relationships, we use \verb+=|+.
BEL statements  can be chained together from the object of the first statement to the subject of the next statement, as shown in~\figref{fig:BEL} for the case of the \ac{MAPK} pathway.

\ac{BEL} provides a number of valuable features for causal modeling.
First, the restriction of \ac{BEL} edges to causal relations implies the topology of the BEL graph can be  reflected in the topology of the causal model.
Second,  the language is expressive enough for humans to manually curate a wide range of biological concepts, but formal enough to serve as a training corpus for \acf{bionlp} competitions~\cite{madan_2019}.
Third, the \ac{BEL} ecosystem is sufficiently mature that causal knowledge represented in other languages can be readily converted to \ac{BEL}~\cite{hoyt_2019,hoyt_2018}.
\begin{center}
    \begin{figure*}
        \begin{small}
            \begin{verbatim}
                kin(p(fplx:RAF)) => kin(p(fplx:MEK))
                kin(p(fplx:MEK)) => kin(p(fplx:ERK))
            \end{verbatim}
        \end{small}
        \caption{\small \textbf{Example BEL statement} The statement details the processes in the MAPK signaling pathway in~\eqref{mapkNet}. The first line states that the kinase activity of RAF directly increases the kinase activity of  MEK. The second line  states that kinase activity of MEK directly increases the kinase activity of ERK. \label{fig:BEL}}
    \end{figure*}
\end{center}    
% This is already described in the intro.
%To bridge the gap between qualitative structured knowledge graphs and quantitative modeling, Gyori {\it et al.} developed the \acf{INDRA} system to automatically assemble a set of causal statements into modeling formalisms including logical causal models\cite{helikar_2012}, agent-based models~\cite{Gundel2018}, probabilisitic graphical models, rule-based models\cite{boutillier_2018,harris_2016}, and \acp{ODE}.
%However, none of these formalisms can support counterfactual inference.
%In this manuscript, we demonstrate an approach for querying a knowledge base such as \ac{INDRA} to export a qualitative causal model represented in the \acl{BEL} and compiling it into to a quantitative \acl{SCM} that can be used to answer counterfactual questions about systems biology and viral pathogenesis.


==> arxiv submission/introduction.tex <==

%% Intro to COVID-19 is a problem. We don't understand it.
%%       * It is novel
%%       * It dysregulates immune reponse in a way that is different from other viruses that we do understand.
%%       * We have lots of questions that modeling can help answer
%%         * How to interpret new data in the light of prior knowledge? 
%%         * What are the determinants of pathogenesis?
%%           * what are the necessary causes of Cytokine storm?
%% * Targets for medical countermeasures
%%           * How cqn we intervene to prevent pathogenesis?


%% Solution:
%%         * Global response connecting experimental and computational biologists
%%         * Rapid response to specific questions

%% Contribution:  Query2BEL and BEL2SCM to quickly answer causal questions.

%% by rapidly interpreting data to knowledge to actionable insight

Each time a cell senses changes in its environment, it marshals a
complex choreography of molecular interactions to initiate an
appropriate response.
When a virus infects the cell, this delicate balance is disrupted and
can result in a cascade of systemic failures leading to disease.
In particular, \acf{sarscov2}, the novel pathogen responsible for the COVID-19 pandemic, has a
complex etiology that differs in subtle and substantial ways from
previously studied viruses.
To make informed decisions about the risk that a new pathogen presents, it is imperative to rapidly predict the determinants of pathogenesis and identify potential targets for medical countermeasures.
Current solutions for this task include systems biology data-driven models, which correlate biomolecular expression to pathogenicity, but cannot go beyond associations in the data to reason about causes of the disease~\cite{pezeshki_2019,pedragosa_2019}. 
Alternatively, hypothesis-driven mathematical models capture causal relations, but are hampered by limited parameter identifiability and predictive power~\cite{nguyen_2016,arazi_2013}.

We argue that counterfactual inference~\cite{pearl2009causal} helps bridge the gap between data-driven and hypothesis-driven approaches. 
It enables questions of the form: ``Had we known the eventual outcome of a patient, what would we have done differently?''
At the heart of counterfactual inference is a formalism known as a \acf{SCM}~\cite{peters2017elements,pearl2009causal}.
It represents prior domain knowledge in terms of causal diagrams, assumes a probability distribution on exogenous variables, and assigns a deterministic function to endogenous variables.
SCM are particularly attractive in systems biology, where structured domain knowledge is extracted from the biomedical literature and is readily available through advances in natural language processing~\cite{Allen2008,McDonald2000,Valenzuela-Escarcega2018}, large-scale automated assembly systems~\cite{gyori2017word}, and semi-automated curation workflows~\cite{hoyt2019}.
This knowledge is curated by multiple organizations~\cite{Cerami2011,Fabregat2018,Kanehisa2017,Perfetto2016,Slenter2018} and stored in structured knowledge bases~\cite{demir_2010,hucka2018systems,le2009systems,Slater2014}.  
It can be brought to bear for answering causal questions regarding SARS-CoV-2. 

This manuscript contributes a three-part algorithm that leverages existing structured biological knowledge to answer counterfactual questions about viral pathogenesis.
Algorithm 1 formalizes biologically relevant questions as queries to an existing causal knowledge graph.
Algorithm 2 converts the query result into a structural causal model.
Algorithm 3  operationalizes the counterfactual inference by interrogating the model with the observed data to estimate a causal effect.

We illustrate the benefits of this approach using two case studies.
Case study 1 illustrates the increased precision of counterfactual estimates, as compared to the ODE- and SDE-based forward simulation, in a situation with known ground truth mechanisms of data generation.
Case study 2 demonstrates the automated construction of an SCM and the value of counterfactual reasoning in novel situations with limited treatment options (as is the case for SARS-CoV-2).
It shows that counterfactual inference enables more precise predictions regarding who would be likely to survive without receiving treatment, who would be likely to die even if they did receive treatment, and who would likely survive only if they received treatment.


